A Side-by-side Comparison of Transformers for English Implicit Discourse Relation Classification

Though discourse parsing can help multiple NLP fields, there has been no wide language model search done on implicit discourse relation classification. This hinders researchers from fully utilizing public-available models in discourse analysis. This work is a straightforward, fine-tuned discourse performance comparison of seven pre-trained language models. We use PDTB-3, a popular discourse relation annotated dataset. Through our model search, we raise SOTA to 0.671 ACC and obtain novel observations. Some are contrary to what has been reported before (Shi and Demberg, 2019b), that sentence-level pre-training objectives (NSP, SBO, SOP) generally fail to produce the best performing model for implicit discourse relation classification. Counterintuitively, similar-sized PLMs with MLM and full attention led to better performance.

==> 050.tex <==
We must admit that there were some necessary simplifications made in terms of experiments. First, we do not report classification accuracies on each implicit sense. In conventional works that deal with a single model \citep{liu2016implicit}, the prediction accuracies of each implicit sense are reported. We omitted this portion in consideration of the large number of PLMs that we deal with. Hence, it must be noted that the final superiority in performance does not equal better classification performance on all class labels. Second, we do not differentiate between intra-sentential implicit and inter-sentential implicit. We report our results on the implicit discourse relations in PDTB-3, which is often characterized by the significantly increased number of intra-sentential implicit in comparison to PDTB-2. There is a possibility that classification performances on these two relation types differ. 

==> 170.tex <==
\begin{table}[ht]
\begin{center}
\footnotesize
\begin{tabular}{lcccc}
\toprule
\textbf{Fold}    & \textbf{Train} & \textbf{Valid} & \textbf{Test} & \textbf{Total}\\ 

\midrule
1                            & 19,412 & 1,641 & 1,607 & 22,660 \\
2                            & 19,410 & 1,574 & 1,641 & 22,625 \\
3                            & 18,992 & 2,025 & 1,574 & 22,591 \\
4                            & 18,844 & 1,729 & 2,025 & 22,598 \\
5                            & 19,779 & 1,134 & 1,729 & 22,642 \\
6                            & 19,549 & 1,939 & 1,134 & 22,622 \\
7                            & 18,470 & 2,197 & 1,939 & 22,606 \\
8                            & 18,502 & 1,927 & 2,197 & 22,626 \\
9                            & 18,697 & 2,004 & 1,927 & 22,628 \\
10                           & 18,975 & 1,657 & 2,004 & 22,636 \\
11                           & 19,417 & 1,580 & 1,657 & 22,654 \\
12                           & 19,359 & 1,723 & 1,580 & 22,662 \\
\midrule
Averaged                     & 19,117 & 1,761 & 1,751 & 22,629 \\
\bottomrule

\end{tabular}
\caption{\# of instances in each fold.}
\vspace{-4mm}
\end{center}
\end{table}
